Decidability of Querying First-Order Theories via Countermodels of Finite Width

We propose a generic framework for establishing the decidability of a wide range of logical entailment problems (briefly called querying), based on the existence of countermodels that are structurally simple, gauged by certain types of width measures (with treewidth and cliquewidth as popular examples). As an important special case of our framework, we identify logics exhibiting width-finite finitely universal model sets, warranting decidable entailment for a wide range of homomorphism-closed queries, subsuming a diverse set of practically relevant query languages. As a particularly powerful width measure, we propose to employ Blumensath's partitionwidth, which subsumes various other commonly considered width measures and exhibits highly favorable computational and structural properties. Focusing on the formalism of existential rules as a popular showcase, we explain how finite partitionwidth sets of rules subsume other known abstract decidable classes but - leveraging existing notions of stratification - also cover a wide range of new rulesets. We expose natural limitations for fitting the class of finite unification sets into our picture and suggest several options for remedy.

==> appendices/treewidth-hyperclique-proof.tex <==

\begin{proof}
Let $T = (V,E)$ be a tree-decomposition of $\inst$ witnessing that $\inst$ has a treewidth of $k$. Then, the countability of $\inst$ implies the countability (and thus, countable degree) of $T$. Therefore, by repeatedly introducing $E$-neighboring copies of nodes, $T$ can be transformed into a full (directed) binary tree $T'=(V',E',\termset)$ with $V'= \{0,1\}^*$, $E'= \{(s,s0), (s,s1) \mid s\in\{0,1\}^*\}$, and $\termset:V'\to 2^{\adom{\inst}}$, which inherits all tree decomposition properties from $T$. The moderate reformulation using the $\termset$ function is necessary due to the introduction of node copies containing identical sets of terms.

Let $\fcn{slot}: \adom{\inst} \to \{0,\ldots,k\}$ be a function that satisfies $\fcn{slot}(t_1)\neq \fcn{slot}(t_2)$ for any $t_1\neq t_2$ with $\{t_1,t_2\} \subseteq \termset(s)$ for some $s\in V'$; note that the existence of such a function is guaranteed by the treewidth bound of $T'$ inherited from $T$. For a tuple $\vt = (t_{1}, \ldots, t_{n})$ of terms, we define $\fcn{slot}(\vt) = (\fcn{slot}(t_{1}), \ldots, \fcn{slot}(t_{n}))$. Moreover, for each domain element $t\in \adom{\inst}$ let $\fcn{pivot}(t)$ denote the node $s \in V'$ with $t \in \termset(s)$ that is closest to the root of $T'$. Also, for each tuple $\vt\in\adom{\inst}^{m}$ with $1 \le m\le \arity{\Sigma}$, let $\fcn{pivot}(\vt)$ denote the node $s\in V'$ that is closest to the root of $T'$ with $t \in \termset(s)$ for each term $t$ occurring in the tuple $\vt$.

For each atom $\rpred(\pi[\vt_1\concat\vt_2]) \in \inst$ and permutation $\pi$ on $\{ 1, \ldots \arity{\rpred} \}$, one of the following three statements must hold for $T'$:

\begin{itemize}
	\item $\fcn{pivot}(\vt_1) = \fcn{pivot}(\vt_2)$, denoted $\vt_1 \approx \vt_2$,
	\item $\fcn{pivot}(\vt_1)$ is an ancestor of $\fcn{pivot}(\vt_2)$, denoted $\vt_1 \prec \vt_2$,
	\item $\fcn{pivot}(\vt_2)$ is an ancestor of $\fcn{pivot}(\vt_1)$, denoted $\vt_2 \prec \vt_1$.
\end{itemize}
 where the the empty tuple is $\prec \vt$ for every nonempty tuple $\vt$. Furthermore, we use $\vec{\downarrow}$ to denote a tuple consisting solely of some number of $\downarrow$ symbols. If we wish to be specific about the number of elements in a tuple $\vec{\downarrow}$, we write $\vec{\downarrow}_{m}$ to indicate that the corresponding tuple contains $m$ occurrences of $\downarrow$.

	For each $1 \le m\le \arity{\Sigma}$, let the finite set $\cols_{m}$ consist of the tuples $(j_1, \ldots, j_m, S)$ with $0 \le j_1, \ldots, j_m \le k$ and $S$ be a subset of
	$$
	\{ (\rpred(\vec{\downarrow}_{m} \hspace{-1ex}{\concat}  \vec{i}), \pi) \mid \rpred \in \Sigma_{>m}, \vec{i}\in\{ 0, \ldots, k\}^{\arity{\rpred} - m}, \text{ and } \pi \text{ is a permutation on } \{ 1, \ldots, \arity{\rpred} \} \}.
	$$
	We set $\cols$ to be the union of the (finitely many) $\cols_{m}$, and provide a description of the process of transforming~$T'$ into an $(\cols,\mathrm{Cnst})$–well-decorated infinite binary tree representing $\inst$. For a node $s$ of $T'$, we define $\fcn{tf}(s)$ as follows:

\begin{itemize}
\item Take a fresh node $v$, decorate it with $\oplus$, and set its two children to be $\fcn{tf}(s0)$ and $\fcn{tf}(s1)$ with $s0$ and $s1$ the two children of $s$ in $T'$. Set $v$ to be the {\em current root} of the transformation.
\item Next, for each $t \in \adom{\inst}$ with $\fcn{pivot}(t)=s$, which we assume are in ascending order by $\fcn{slot}(t)$ (there are at most $k+1$ of such terms), do the following:
    \begin{enumerate}
    \item Take a fresh node $v'$, decorate it with $\oplus$, and make the current root $v$ its left child and let its right child be a fresh node $u$ decorated with $\precol_{\origcol \to (j, S)}$ and having a fresh left child node $z$ (i.e. $z$ is set as the left child of $u$), which is decorated by $t$ if $t \in \mathrm{Cnst}$, or $\const{*}$ otherwise, and where $j = \fcn{slot}(t)$ and $S$ contains:
        \begin{itemize}
%        \item[$\circ$] \textcolor{gray}{all $\rpred(\downarrow)$ with $\rpred(t) \in \inst$ and all $\rpred(\downarrow,\downarrow)$ with $\rpred(t,t) \in \inst$, } \textcolor{thomas}{Should be subsumed by the next entry and case $m=2$ later on, by the assumption that the empty tuple of terms is always a ``pivotal ancestor'' of every tuple.}
        \item[$\circ$] all $(\rpred(\downarrow,\vec{i}), \pi)$ with $\rpred(\pi[t\concat\vt']) \in \inst$ for some $\vt' \in \adom{\inst}^{\arity{\rpred} - 1}$ with $\fcn{slot}(\vt')=\vec{i}$ and where either $\vt'\prec t$, or if $\vt'\approx t$, then $\min\{i \ | \ i \in \vec{i}\}>j$.
        \end{itemize}
    \item Build a chain $P$ of nodes decorated with $\pcadd$ and $\precol$ predicates to reflect the following set of operations:
        \begin{itemize}
        \item[$\circ$] for every unary colorset containing $(j,S)$, for which $S$ contains some $\rpred(\downarrow)$, perform %$\fcadd_{(j,S), \rpred}$ and then 
        $\frecol_{(j,S)\to \{ (j,S \setminus \{\rpred(\downarrow)\}) \} \cup \{ \rpred \}}$,
        \item[$\circ$] for any two colors $(j,S)$ and $(\vec{i},S')$ where $m  =\arity{\vec{i}, S'}$, for which $S'$ contains some $(\rpred(\vec{\downarrow}_m,j), \pi)$, perform $\fcadd_{(\vec{i},S')(j,S), \rpred}^{\pi}$ and immediately afterward perform $\frecol_{(\vec{i},S')\to(\vec{i},S' \setminus \{(\rpred(\vec{\downarrow},j), \pi)\})}$.
        \end{itemize}
    \item Set the current root to be the highest node of $P$ and set $v'$ to be the child of the lowest node of $P$.
    \item Denote the current node by $v^{1}$.
    \end{enumerate}
\item Next, assume the current node to be $v^{m-1}$. Go through all $\vt \in \adom{\inst}^{m}$ with $\fcn{pivot}(\vt)=s$, which we assume are in ascending order induced lexicographically by $\fcn{slot}(\vt)$ (there are at most $(k+1)^{m}$ of such terms) and build the following chain $P$:
\begin{enumerate}
	\item Start building the chain $P$ as a chain of nodes decorated with $\pcadd$ reflecting for every $(\vec{j}, S)\in \cols_{m-1}$ and $(j, S')\in \cols_1$ the operations $\fcadd_{(\vec{j}, S)(j, S'), (\vec{j}\concat j, S'')}$ where $\vec{j} = \fcn{slot}(t_1, \ldots, t_{m-1})$, $j = \fcn{slot}(t_m)$ and $S''$ contains all $(\rpred(\vec{\downarrow}_m\! \concat \ \vec{i}), \pi)$ such that $\rpred(\pi[\vt\concat\vt'])\in\inst$ for some $\vt'$ from $\adom{\inst}$ with $\fcn{slot}(\vt') = \vec{i}$ and where either $\vt'\prec \vt$, or  if $\vt'\approx \vt$, then $\min{\vec{i}} > \max{\vec{j}}$.
	\item Extend the chain $P$ by adding nodes decorated with $\pcadd$ and $\precol$ predicates to reflect the following set of operations:
	\begin{itemize}
		\item[$\circ$] for every colorset of $< m$-ary colors containing $(\vec{j},S)$, for which $S$ contains some $\rpred(\vec{\downarrow})$, perform %$\fcadd_{(j,S), \rpred}$ and then 
		$\frecol_{(\vec{j},S)\to \{ (\vec{j},S \setminus \{\rpred(\downarrow)\}) \} \cup \{ \rpred \}}$,
		\item[$\circ$] for any two colors $(\vec{j},S)$ and $(\vec{i},S')$, for which $S'$ contains some $(\rpred(\vec{\downarrow}_{\length{\vec{i}}}\concat\vec{j}), \pi)$, perform $\fcadd_{(\vec{i},S')(\vec{j},S), \rpred}^{\pi}$ and immediately afterward $\frecol_{(\vec{i},S')\to(\vec{i},S' \setminus \{(\rpred(\vec{\downarrow}_{\length{\vec{i}}}\concat\vec{j}), \pi)\})}$.
	\end{itemize}
	\item Set the current root to be the highest node of $P$ and set $v^{m-1}$ to be the child of the lowest node of $P$.
	\item Denote the current node by $v^{m}$.
\end{enumerate}
\end{itemize}

To obtain $\fcn{tf}(s)$, take the resulting decorated tree and extend the resulting tree to an infinite binary tree by adding missing elements and decorating them with $\pred{Void}$.

Finally, take the root $\varepsilon$ of $T'$ and obtain $\fcn{tf}(\varepsilon)$ based on the above procedure. After, add nodes decorated with $\pcadd_\rpred^{\pi}$ above the root of $\fcn{tf}(\varepsilon)$ (in any order), where $\pi : \emptyset \to \emptyset$ is the empty permutation and $\rpred \in \Sigma$ is a nullary predicate with $\rpred \in \inst$. Once again, add in any missing nodes to create an infinite binary tree and decorate such nodes with $\pred{Void}$. The resulting $(\cols,\mathrm{Cnst})$-well-decorated tree represents $\inst$.
\end{proof}


==> figure1.tex <==

\begin{figure*}

\hspace{-2ex}

\begin{center}

\remarkstart
$(\newconst{a} \oplus_{\{ \unradd{\origcol_{2}}{\epred}^{0}, \unradd{\origcol_{2}}{\epred}^{1}, \radd{\origcol_1}{\origcol_1}{\{1\}}{\epred}, \radd{\origcol_1}{\origcol_1}{\{2\}}{\epred} \}} \newconst{b}) \oplus_{\{\radd{\origcol_1}{\lambda}{\{1\}}{\epred}\}} (\newconst{c} \oplus_{\{\recol{\origcol_{1}}{\lambda}^0, \recol{\origcol_{1}}{\lambda}^1\}} \newanon)$
\color{black}
\\[1ex]
\!\scalebox{0.7689}{
\begin{tikzpicture}[level/.style={sibling distance=60mm/#1, level distance=15mm}]
%[
%    level 1/.style={sibling distance=40mm, level distance=10mm},
%    level 2/.style={sibling distance=35mm, level distance=10mm},
%    level 3/.style={sibling distance=30mm, level distance=10mm},
%    level 4/.style={sibling distance=20mm, level distance=10mm},
%    level 5/.style={sibling distance=15mm, level distance=10mm}
%]


\node [label={[label distance=-4pt]0:$ \ : \ \radd{\origcol_1}{\lambda}{\{1\}}{\epred}  $}] (a){$\varepsilon$}
  child {node [label={[label distance=-4pt]0: $ \ : \  \unradd{\origcol_{2}}{\epred}^{0}, \unradd{\origcol_{2}}{\epred}^{1}, $}] (n0) {$0$}
        child {node [label={[label distance=-4pt]0:$ \ : \ \newconst{a}$}] (n00) {$00$}
                    child {node [] (n00000) { }
                    edge from parent [-,color=black,line width=1pt,path fading=South] node [] {}
                    }
                    child {node [opacity=0.2,path fading=South,color=gray!60] (n00001) { }
                    edge from parent [-,color=gray!60,line width=1pt,path fading=South] node [] {}
                    }
                edge from parent [-,color=black,line width=1pt] node [] {}
        } %end 00
        child {node [label={[label distance=-4pt]0:$ \ : \ \newconst{b}$}] (n01) {$01$}
        child {node [opacity=0.2] (n010) { }
        edge from parent [-,color=black,line width=1pt,path fading=South] node [] {}
            } %end 010
        child {node [opacity=0.2] (n011) { }
        edge from parent [-,color=gray!60,line width=1pt,path fading=South] node [] {}
            } %end 011
    edge from parent [-,color=gray!60,line width=1pt] node [] {}
    } %end 01
edge from parent [-,line width=1pt] node [] {}
} %end 0
child {node [label={[label distance=-4pt]0:$ \ : \ \recol{\origcol_{1}}{\lambda}^0,$}] (n0) {$1$}
    child {node [label={[label distance=-4pt]0:$ \ : \ \newconst{c}$}] (n00) {$10$}
        child {node [] (n000) { }
        edge from parent [-,color=black,line width=1pt,path fading=South] node [] {}
        } %end 000
        child {node [opacity=0.2,path fading=South,color=gray!60] (n001) { }
            edge from parent [-,color=gray!60,line width=1pt,path fading=South] node [] {}
        } %end 001
        edge from parent [-,color=black,line width=1pt] node [] {}
        } %end 00
    child {node [label={[label distance=-4pt]0:$ \ : \ \newanon$}] (n01) {$11$}
        child {node [opacity=0.2] (n110) { }
        edge from parent [-,color=black,line width=1pt,path fading=South] node [] {}
            } %end 010
        child {node [opacity=0.2] (n111) { }
        edge from parent [-,color=gray!60,line width=1pt,path fading=South] node [] {}
            } %end 011
    edge from parent [-,color=gray!60,line width=1pt] node [] {}
    } %end 11
edge from parent [-,color=gray!60,line width=1pt] node [] {}
}; %end 1


\node[] (z) [left=of a, xshift=-1.5cm,yshift=-0.75cm,label={[label distance=0pt]135:\scalebox{2}{$\mathcal{T} \ =$}}] { };
%{$\underset{ \ \rotatebox{0}{=}}{\mathcal{T} \quad \ }$}}] { };

\node[] (z3) [below=of a, xshift=-0.65cm,yshift=-1.15cm,label={
{ $\radd{\origcol_1}{\origcol_1}{\{1\}}{\epred}, \radd{\origcol_1}{\origcol_1}{\{2\}}{\epred}$}}] { };

\node[] (z4) [below=of a, xshift=4.75cm,yshift=-1.15cm,label={
{ $\recol{\origcol_{1}}{\lambda}^1$}}] { };

%\node[] (z3) [below=of n00000, xshift=4cm,yshift=0cm,label={$\mathit{Ins}_{1} = \{\unradd{\origcol_{2}}{\epred}^{0}, \unradd{\origcol_{2}}{\epred}^{1}, \radd{\origcol_1}{\origcol_1}{\{1\}}{\epred}, \radd{\origcol_1}{\origcol_1}{\{2\}}{\epred}, \radd{\origcol_1}{\origcol_1}{\{1,2\}}{\epred}\}$}] { };

%\node[] (z4) [below=of n00000, xshift=2.45cm,yshift=-0.75cm,label={$\mathit{Ins}_{2} = \{\recol{\origcol_{1}}{\lambda}^0, \recol{\origcol_{1}}{\lambda}^1 \}$}] { };

%\node[] (z5) [below=of n00000, xshift=1.5cm,yshift=-1.5cm,label={$\mathit{Ins}_{3} = \{\radd{\origcol_1}{\origcol_1}{\{1\}}{\epred}\}$}] { };
     
     
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% Graph / Clique
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[] (x1) [left=of a, xshift=10cm,yshift=-0.5cm,label={[label distance=0pt]45:$ $}] {$\const{b}$};
\node[] (x2) [below=of x1, xshift=0mm,yshift=-15mm,label={[label distance=0pt]-45:$ $}] {$\const{a}$};
\node[] (x3) [right=of x1, xshift=15mm] %[right=of x1, xshift=15mm,label={[label distance=0pt]45:$\lambda$}] 
 {$\const{c}$};
\node[] (x4) [right=of x2, xshift=15mm] %[right=of x2, xshift=15mm,label={[label distance=0pt]-45:$\lambda$}] 
 {$11$};

    \draw [->](x1) to [out=180,in=90,looseness=8] node[midway,label={[label distance=0pt]180:$\pred{E}$}] {} (x1);
    \draw [->](x1) to [bend left] node[midway,label={[label distance=0pt]0:$\pred{E}$}] {} (x2);
    \draw [->](x2) to [out=180,in=270,looseness=8] node[midway,label={[label distance=0pt]180:$\pred{E}$}] {} (x2);
    \draw [->](x2) to [bend left] node[midway,label={[label distance=0pt]180:$\pred{E}$}] {} (x1);
    
    \draw[->,color=black] (x1) -- (x3) node [midway,label={[label distance=0pt]90:$\pred{E}$}] {};
    \draw[->,color=black] (x2) -- (x3) node [midway,xshift=5pt,label={[label distance=5pt]90:$\pred{E}$}] {};
    \draw[->,color=black] (x1) -- (x4) node [midway,xshift=5pt,label={[label distance=5pt]-90:$\pred{E}$}] {};
    \draw[->,color=black] (x2) -- (x4) node [midway,label={[label distance=0pt]-90:$\pred{E}$}] {};

\node[] (z2) [right=of x3, xshift=1cm,yshift=-2cm,label={[label distance=0pt]135:\scalebox{2}{$= \ \instance^{\mathcal{T}}$}}] { };
\end{tikzpicture}
}
\end{center}

\vspace{-4ex}

\caption{\remarkstart Top: Term describing the assembly of a finite structure. \color{black} 
	Left: Corresponding well-decorated binary tree $\mathcal{T}$ with $\pred{Succ}_{0}$ and $\pred{Succ}_{1}$ represented as black (left) and gray (right) edges, respectively; all non-displayed nodes are not decorated. 
%
 Right: Graphical depiction of the instance $\inst^{\mathcal{T}}$ generated by $\mathcal{T}$, where $\cols = \{\origcol_{1},\origcol_{2}, \lambda\}$, $\sig = \{\pred{E}\}$, $\arity{\origcol_{1}} = \arity{\lambda} = 1$,  $\arity{\origcol_{2}} = \arity{\pred{E}} = 2$, and $\mathrm{Cnst} = \{\const{a},\const{b},\const{c}\}$. $\mathcal{T}$ encodes the syntax tree of the ``assembly expression'' shown above $\inst^{\mathcal{T}}$.
}
\label{fig:well-decotrated-tree-example}
\end{figure*}


==> figure2.tex <==

\begin{figure}[t]
\vspace{-1ex}	
\hspace{-1ex}
\scalebox{0.8}{	
\begin{tikzpicture}[
		Dotted/.style={% https://tex.stackexchange.com/a/52856/194703
			dash pattern=on 0.1\pgflinewidth off #1\pgflinewidth,line cap=round,
			shorten >=#1\pgflinewidth/2,shorten <=#1\pgflinewidth/2},
		Dotted/.default=3]
		
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Well Decorated Tree
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


		
\node[] [] (n) [label={[label distance=-2pt]0:$ $}] {$\varepsilon$};
    %LEVEL 1 LEFT
    \node[] [] (n0) [below left=of n,xshift=0cm,yshift=-.1cm,label={[label distance=-2pt]0:$: \newanon$}] {$0$};
    \draw[-,color=black,line width=1pt] (n) -- (n0) node [] { };
	    \node[] [] (n00) [below left = of n0,xshift=0mm] { };
		\draw[-,color=black,line width=1pt,path fading=South] (n0) -- (n00) node [] {};
	    \node[] [] (n01) [below = of n0,xshift=0mm] { };
		\draw[-,color=gray!60,line width=1pt,path fading=South] (n0) -- (n01) node [] {};
	%LEVEL 1 RIGHT
    \node[] [] (n1) [below=of n,yshift=-27.7mm,label={[label distance=-2pt]0:$ $}] {$1$};
    \draw[-,color=gray!60,line width=1pt] (n) -- (n1) node [] { };
        \node[] [] (n10) [below left=of n1,xshift=.1cm,yshift=-0.9cm,label={[label distance=-2pt]0:$: \newanon$}] {$10$};
        \draw[-,color=black,line width=1pt] (n1) -- (n10) node [] { };
	        \node[] [] (n100) [below left = of n10] { };
		    \draw[-,color=black,line width=1pt,path fading=South] (n10) -- (n100) node [] {};
	        \node[] [] (n101) [below = of n10] { };
		    \draw[-,color=gray!60,line width=1pt,path fading=South] (n10) -- (n101) node [] {};
	    \node[] [] (n11) [below = of n1,yshift=-17mm] {$\vdots$};
	    \draw[-,color=gray!60,line width=1pt] (n1) -- (n11) node [] {};
	    %\draw[-,color=gray!60,line width=1pt,path fading=South] (n1) -- (n11) node [] {};
	    %\draw[-,color=gray!60,line width=1pt] (n1) -- (n11) edge [dotted] ($(n11)!3.1cm!(n1)$);
	    


		
\node[] (T) [left=of n, xshift=0.5cm,yshift=-0.5cm,label={[label distance=0pt]135:\scalebox{2}{$\mathcal{T} \ \rotatebox{0}{=}$}}] { };	
		
		
		
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Expressions & Instances
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	

\node[] (IT) [right=of n, xshift=8.75cm,yshift=0.80cm,label={[label distance=0pt]135:\scalebox{2}{$\cong \inst^\mathcal{T}$}}] { }; %{$ \cong \inst^\mathcal{T}$}}] { };

%\node[] (IT) [right=of n, xshift=8.25cm,yshift=1.25cm,label={[label distance=0pt]135:\scalebox{2}{$\underset{\rotatebox{45}{ $\cong$ }}{\inst^\mathcal{T}}$}}] { }; %{$ \cong \inst^\mathcal{T}$}}] { };


%%%%%%%%%%%%%	
%%%Eighth LINE
%%%%%%%%%%%%%	
		\node[] (h1) [right=of n, xshift=3.5cm, yshift=.65cm, label={[label distance=-2pt]-90:$\kappa$}, yshift=-0pt] %xshift=40pt,
		{$0$};
		\node[] (h2) [right=of h1,label={[label distance=-2pt]-90:$\kappa$}] {$1$};
		\node[] (h3) [right=of h2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
		\node[] (h5) [right=of h3,xshift=-1cm] {$\cdots$};
		\node[] (h6) [left=of h5,xshift=-4cm] {$\radd{\origcol_{1}}{\lambda}{\{1\}}{\rpred} \ \ $};
		\node[] (h8) [left=of h1,label={[label distance=-2pt]-90:$\origcol_{1}$}] {$-1$};
		
		\draw[->] (h1) -- (h2) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		\draw[-,transform canvas={yshift=6.pt,xshift=-12pt}] (h1) -- ($(h1)!3.06cm!(h3)$) node [] {};
		\draw[->] (h2) -- (h3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};

		\node[] (h9) [right=of h8,xshift=-.05cm] { };
		\node[] (h10) [left=of h1,xshift=-.05cm] { };

\begin{scope}[local bounding box=only paths]
\draw[fill=gray!25, fill opacity=.7] (h8) to[out=45,in=135] (h3);
  \draw[fill=gray!25, fill opacity=.7] (h8) to[out=45,in=135] (h2);
  \draw[fill=white] (h8) to[out=45,in=135] (h1); 
   \filldraw [white, line width=.45cm] (h9) -- (h10);
\end{scope}


\node[] [] (R) [above=of h1,yshift=-1cm,xshift=.2cm]{$\pred{R}$};
\node[] [] (R) [above=of h2,yshift=-.8cm,xshift=-.1cm]{$\pred{R}$};
		
		
		
%%%%%%%%%%%%%			
%%%Seventh LINE
%%%%%%%%%%%%%	
		\node[] (g1) [below= of h1, label={[label distance=-2pt]-90:$\kappa$},yshift=10pt] %,xshift=40pt] 
		{$0$};
		\node[] (g2) [right=of g1,label={[label distance=-2pt]-90:$\kappa$}] {$1$};
		\node[] (g3) [right=of g2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
%		\node[] (g4) [right=of g3,label={[label distance=-2pt]-90:$\kappa$}] {$3$};
		\node[] (g5) [right=of g3,xshift=-1cm] {$\cdots$};
		\node[] (g6) [left=of g5,xshift=-4cm] {$\recol{\mu}{\kappa}^{1} \quad$}; % {$\const{*} \oplus_{\mathit{Ins}_{1}} E \ \ $};
		\node[] (g8) [left=of g1,label={[label distance=-2pt]-90:$\origcol_{1}$}] {$-1$};
		
		\draw[->] (g1) -- (g2) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		\draw[->] (g2) -- (g3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		

%%%%%%%%%%%%%		
%%%Sixth LINE
%%%%%%%%%%%%%	
		\node[] (f1) [below= of g1, label={[label distance=-2pt]-90:$\mu$},yshift=10pt] {$0$};  %,xshift=40pt] {$0$};
		\node[] (f2) [right=of f1,label={[label distance=-2pt]-90:$\kappa$}] {$1$};
		\node[] (f3) [right=of f2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
		\node[] (f5) [right=of f3,xshift=-1cm] {$\cdots$};
		\node[] (f6) [left=of f1,label={[label distance=-2pt]-90:$\origcol_{1}$}] {$-1$};
		
		\draw[->] (f1) -- (f2) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		\draw[->] (f2) -- (f3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		
		
%%%%%%%%%%%%%	
%%%Dots / Separation
%%%%%%%%%%%%%	
%\node[] [] (dots) [below=of f2,yshift=.6cm]{$\vdots$};
		
		
		
%%%%%%%%%%%%%			
%%%Fifth LINE
%%%%%%%%%%%%%	
		\node[] [] (e1) [below=of f1, label={[label distance=-2pt]-90:$\mu$}, yshift=7pt] {$0$};
		\node[] (e2) [right=of e1,label={[label distance=-2pt]-90:$\kappa$}] {$1$};
		\node[] (e3) [right=of e2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
		\node[] (e4) [right=of e3,label={[label distance=-2pt]-90:$ $}] {$ $};
		\node[] (e5) [right=of e3,xshift=-1cm] {$\cdots$};
		\node[] (e6) [left=of e4,xshift=-4.5cm] {$\recol{\origcol_{1}}{\mu}^{0} \qquad $};
		
		\draw[->] (e1) -- (e2) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		\draw[->] (e2) -- (e3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};

	
		
%%%%%%%%%%%%%			
%%%fourth LINE
%%%%%%%%%%%%%	
		\node[] [] (d1) [below=of e1, label={[label distance=-2pt]-90:$\origcol_{1}$}, yshift=7pt] {$0$};
		\node[] (d2) [right=of d1,label={[label distance=-2pt]-90:$\kappa$}] {$1$};
		\node[] (d3) [right=of d2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
		\node[] (d4) [right=of d3,label={[label distance=-2pt]-90:$ $}] {$ $};
		\node[] (d5) [right=of d3,xshift=-1cm] {$\cdots$};
		\node[] (d6) [left=of d4,xshift=-4.5cm] {$\recol{\mu}{\kappa}^{1} \qquad \phantom{)}$};
		
		\draw[->] (d1) -- (d2) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		\draw[->] (d2) -- (d3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};



		
%%%%%%%%%%%
%%%third LINE
%%%%%%%%%%%
		\node[] [] (c1) [below=of d1, label={[label distance=-2pt]-90:$\origcol_{1}$}, yshift=7pt] {$0$};
		\node[] (c2) [right=of c1,label={[label distance=-2pt]-90:$\mu$}] {$1$};
		\node[] (c3) [right=of c2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
		\node[] (c4) [right=of c3,label={[label distance=-2pt]-90:$ $}] {$ $};
		\node[] (c5) [right=of c3,xshift=-1cm] {$\cdots$};
		\node[] (c6) [left=of c4,xshift=-4.5cm] {$\cadd{\origcol_{1}}{\mu}{\{1\}}{\lambda} \qquad \phantom{)}$};
		
		\draw[->] (c1) -- (c2) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};
		\draw[->] (c2) -- (c3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};

		


%%%%%%%%%%
%%%second LINE
%%%%%%%%%%%%
		\node[] [] (a1) [below = of c1, label={[label distance=-2pt]-90:$\origcol_{1}$}, yshift=8.3pt] {$0$};
		\node[] (a2) [right=of a1,label={[label distance=-2pt]-90:$\mu$}] {$1$};
		\node[] (a3) [right=of a2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
		\node[] (a4) [right=of a3,label={[label distance=-2pt]-90:$ $}] {$ $};
		\node[] (a5) [right=of a3,xshift=-1cm] {$\cdots$};
		\node[] (a6) [left=of a4,,xshift=-4.5cm] { }; %{$\const{*} \oplus E\phantom{)))} \ \ $};
		
		\draw[->] (a2) -- (a3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};


		
%%%%%%%%
%%%first LINE
%%%%%%%%
%		\node[] [] (z1) [below = of a1, yshift=7pt] {$\phantom{0}$};
%		\node[] (z2) [right=of z1,label={[label distance=-2pt]-90:$\mu$}] {$1$};
%		\node[] (z3) [right=of z2,label={[label distance=-2pt]-90:$\kappa$}] {$2$};
%		\node[] (z4) [right=of z3,label={[label distance=-2pt]-90:$ $}] {$ $};
%		\node[] (z5) [right=of z3,xshift=-1cm] {$\cdots$};
%		\node[] (z6) [left=of z4,xshift=-4.5cm] {}; % {$E \phantom{)))} \ \  $};
		
%		\draw[->] (z2) -- (z3) node [midway,label={[label distance=-2pt]-90:$\lambda$}] {};


%%%%%%%%%%	
%%%Dots
%%%%%%%%%
	
\node[] [] (dots) [below=of a2,yshift=.75cm, xshift=0cm]{$\vdots$};


%%%%%%%%%%
%%BRACKETS
%%%%%%%%%%	

\node[] (B1) [left=of h1, xshift=-2.5cm,yshift=-1.85cm,label={[label distance=0pt]135:\scalebox{1.5}[2]{$\bigg\{$}}] { };

%\node[] (B11) [left=of B1, xshift=.5cm, yshift=.7cm, label={[label distance=0pt]135:\scalebox{1.2}[1.2]{$\mathit{Ins}_{1} = $}}] { };

\node[] (B2) [below=of B1, xshift=0cm,yshift=-3.8cm,label={[label distance=0pt]135:\scalebox{1.5}[3]{$\Bigg\{$}}] { };

%\node[] (B21) [left=of B2, xshift=.5cm, yshift=1.5cm, label={[label distance=0pt]135:\scalebox{1.2}[1.2]{$\mathit{Ins}_{2} = $}}] { };
		
\end{tikzpicture}
}
	
\vspace{-2ex}	
\caption{\!\!Right: Assembly process of instance $\inst_{\mathrm{tern}}= \{ \rpred(-1,n,n{+}1) \mid n{\in} \mathbb{N} \}$ (each integer from $\{-1\} \cup \mathbb{N}$ stands for a null), to be read bottom-up. We use the colors $\origcol_{1}, \kappa, \mu, \lambda \in \cols$ with $\arity{\origcol_{1}} = \arity{\kappa} = \arity{\mu} = 1$ and $\arity{\lambda} = 2$. We set $\cnst = \emptyset$ and $\Sigma = \{\pred{R}\}$ with $\arity{\pred{R}} = 3$. 
Left: Corresponding well-decorated tree $\mathcal{T}$, encoding application of operations during assembly. $\pred{Succ}_{0}$ and $\pred{Succ}_{1}$ are represented as black (left) and gray (right) edges, respectively. $\inst_{\mathrm{tern}}$ is assembled in two phases: first, construct an infinite line in a non-well-founded manner by repeating the operations shown to the right of the null $1$ for all nulls of the form $1^{n}$ occurring in $\mathcal{T}$. This first phase of the assembly process consists of an infinite repetition of the following three steps: given a line with initial element $n{+}1$, (1) add an additional element $n$ colored with $\origcol_{1}$, (2) connect $n$ to the $\mu$-colored element $n{+}1$ via the binary color $\lambda$, and (3) recolor $n{+}1$ to $\kappa$ and $n$ to $\mu$. The second phase of the assembly process, shown as the top three steps/lines on the right, is encoded in the root of $\mathcal{T}$: introduce a fresh element, denoted $-1$, and connect it to each consecutive pair of natural numbers $n$ and $n{+}1$ in $\inst$ via the ternary predicate $\pred{R}$. 
%Since our instance $\inst^{\mathcal{T}}$ is defined relative to the signature $\sig = \{\pred{R}\}$, $\inst^{\mathcal{T}}$ is indeed isomorphic to $\inst_{\mathrm{tern}}$.
}
\label{fig:infinite-line-example}
\vspace{-2ex}
\end{figure}

